Foundations of Total Functional Data-Flow Programming

The field of declarative stream programming (discrete time, clocked synchronous, modular, data-centric) is divided between the data-flow graph paradigm favored by domain experts, and the functional reactive paradigm favored by academics. In this paper, we describe the foundations of a framework for unifying functional and data-flow styles that differs from FRP proper in significant ways: It is based on set theory to match the expectations of domain experts, and the two paradigms are reduced symmetrically to a low-level middle ground, with strongly compositional semantics. The design of the framework is derived from mathematical first principles, in particular coalgebraic coinduction and a standard relational model of stateful computation. The abstract syntax and semantics introduced here constitute the full core of a novel stream programming language.

==> eptcsdata.tex <==
\providecommand{\firstpage}{143}
\providecommand{\publicationstatus}{N.R. Krishnaswami and P.B. Levy (Eds.): \\Mathematically Structured Functional Programming 2014 (MSFP 2014). \\
EPTCS 153, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.153.10}{10.4204/EPTCS.153.10}}
\pdfoutput=1

